VIEScore: Towards Explainable Metrics for Conditional Image Synthesis Evaluation

In the rapidly advancing field of conditional image generation research, challenges such as limited explainability lie in effectively evaluating the performance and capabilities of various models. This paper introduces VIEScore, a Visual Instruction-guided Explainable metric for evaluating any conditional image generation tasks. VIEScore leverages general knowledge from Multimodal Large Language Models (MLLMs) as the backbone and does not require training or fine-tuning. We evaluate VIEScore on seven prominent tasks in conditional image tasks and found: (1) VIEScore (GPT4-o) achieves a high Spearman correlation of 0.4 with human evaluations, while the human-to-human correlation is 0.45. (2) VIEScore (with open-source MLLM) is significantly weaker than GPT-4o and GPT-4v in evaluating synthetic images. (3) VIEScore achieves a correlation on par with human ratings in the generation tasks but struggles in editing tasks. With these results, we believe VIEScore shows its great potential to replace human judges in evaluating image synthesis tasks.

==> backup.tex <==
\begin{table}[!t]
\centering
\scalebox{0.85}{
\begin{tabular}{l|ccc}
\toprule
M-Sie:MLLM & M-H$^{SC}_{\text{corr}}$ & M-H$^{PQ}_{\text{corr}}$ & M-H$^{O}_{\text{corr}}$ \\
\midrule
\multicolumn{4}{c}{Text-guided Image Generation (5 models)} \\
Human Raters & 0.5044 & 0.3640 & 0.4652 \\
\midrule
GPT-4v (0-shot) & \colorbox{green}{0.4885} &  \colorbox{green}{0.2379} & \colorbox{green}{0.4614} \\
GPT-4v (1-shot) & \colorbox{green}{0.4531} & 0.1770 & \colorbox{green}{0.3801} \\
LLaVA (0-shot) &  0.1809 &  0.0306 &  0.1410 \\
LLaVA (1-shot) & 0.1789 & -0.0020 & 0.1309 \\
\midrule
\multicolumn{4}{c}{Mask-guided Image Editing (4 models)} \\
Human Raters & 0.5390 & 0.5030 & 0.4981 \\
\midrule
GPT-4v (0-shot) & \colorbox{green}{0.4508} &  0.2859 & \colorbox{green}{0.4069} \\
GPT-4v (1-shot) & \colorbox{green}{0.4088} & 0.2352 & \colorbox{green}{0.3810} \\
LLaVA (0-shot) &  0.1180 &  -0.0531 &  0.0675 \\
LLaVA (1-shot) & 0.1263 & -0.0145 & 0.1040 \\
\midrule
\multicolumn{4}{c}{Text-guided Image Editing (8 models)} \\
Human Raters & 0.4230 & 0.5052 & 0.4184 \\
\midrule
GPT-4v (0-shot) &  0.2610 & \colorbox{green}{0.4274} &  0.2456 \\
GPT-4v (1-shot) & 0.2428 & 0.3402 & 0.2279 \\
LLaVA (0-shot) & 0.0448 & 0.0583 &  0.0273 \\
LLaVA (1-shot) & 0.0185 & -0.0107 & 0.0258 \\
\midrule
\multicolumn{4}{c}{Subject-driven Image Generation (4 models)} \\
Human Raters & 0.4780 & 0.3565 & 0.4653 \\
\midrule
GPT-4v (0-shot) & \colorbox{green}{0.3979} &  0.1903 & \colorbox{green}{0.3738} \\
GPT-4v (1-shot) & 0.2757 & \colorbox{green}{0.2261} & 0.2753 \\
LLaVA (0-shot) &  0.0326 &  -0.0303 &  0.1219 \\
LLaVA (1-shot) & 0.1334 & 0.0858 & 0.1248 \\
\midrule
\multicolumn{4}{c}{Subject-driven Image Editing (3 models)} \\
Human Raters & 0.4887 & 0.2986 & 0.4747 \\
\midrule
GPT-4v (0-shot) & \colorbox{green}{0.3274} &  \colorbox{green}{0.2960} &  0.1507 \\
GPT-4v (1-shot) & -0.0255 & \colorbox{green}{0.1572} & -0.0139 \\
LLaVA (0-shot) &  0.0360 &  -0.0073 &  0.0168 \\
LLaVA (1-shot) & 0.0587 &  -0.0249 & 0.0309 \\
\midrule
\multicolumn{4}{c}{Multi-concept Image Composition (3 models)} \\
Human Raters & 0.5927 & 0.5145 & 0.5919 \\
\midrule
GPT-4v (0-shot) & 0.3209 & 0.3025 & 0.3346 \\
GPT-4v (1-shot) & 0.1859 & 0.1185 & 0.1918 \\
LLaVA (0-shot) &  0.1022 &  0.1194 &  0.1070 \\
LLaVA (1-shot) & 0.0828 & 0.0379 & 0.0293 \\
\midrule
\multicolumn{4}{c}{Control-guided Image Generation (2 models)} \\
Human Raters & 0.5443 & 0.5279 & 0.5307 \\
\midrule
GPT-4v (0-shot) & \colorbox{green}{0.4360} & \colorbox{green}{0.4975} & \colorbox{green}{0.3999} \\
GPT-4v (1-shot) & 0.3892 & \colorbox{green}{0.4132} & \colorbox{green}{0.4237} \\
LLaVA (0-shot) &  0.2207 &  0.1060 &  0.1679 \\
LLaVA (1-shot) & 0.1121 & 0.0247 & 0.0416 \\
\bottomrule
\end{tabular} }
\caption{Correlations in each task. We highlight
correlations less than 0.15 difference to human correlation.}
\label{tab:result}
\end{table}



\begin{table}[!t]
\centering
\scalebox{0.85}{
\begin{tabular}{l|ccc}
\toprule
Metric & M-H$^{SC}_{\text{corr}}$ & M-H$^{PQ}_{\text{corr}}$ & M-H$^{O}_{\text{corr}}$ \\
\midrule
\multicolumn{4}{c}{Text-guided Image Generation (5 models)} \\
Human Raters & 0.5044 & 0.3640 & 0.4652 \\
\midrule
\colorbox{yellow}{M-Sie:GPT-4v} & 0.4885 &  0.2379 & 0.4614 \\
CLIP-Score & -0.0817 & -0.0114 & -0.0881 \\
\midrule
\multicolumn{4}{c}{Mask-guided Image Editing (4 models)} \\
Human Raters & 0.5390 & 0.5030 & 0.4981 \\
\midrule
\colorbox{yellow}{M-Sie:GPT-4v} & 0.4508 &  0.2859 & 0.4069 \\
LPIPS & -0.1012 & 0.0646 & -0.0694 \\
\midrule
\multicolumn{4}{c}{Text-guided Image Editing (8 models)} \\
Human Raters & 0.4230 & 0.5052 & 0.4184 \\
\midrule
\colorbox{yellow}{M-Sie:GPT-4v} & 0.2610 & 0.4274 &  0.2456 \\
LPIPS & 0.0956 & 0.2504 & 0.1142 \\
\midrule
\multicolumn{4}{c}{Subject-driven Image Generation (4 models)} \\
Human Raters & 0.4780 & 0.3565 & 0.4653 \\
\midrule
M-Sie:GPT-4v & 0.3979 &  0.1903 & 0.3738 \\
\colorbox{yellow}{DINO} & 0.4160 & 0.1206 & 0.4246 \\
CLIP-I & 0.2961 & 0.1694 & 0.3058 \\
\midrule
\multicolumn{4}{c}{Subject-driven Image Editing (3 models)} \\
Human Raters & 0.4887 & 0.2986 & 0.4747 \\
\midrule
M-Sie:GPT-4v & 0.3274 &  0.2960 &  0.1507 \\
\colorbox{yellow}{DINO} & 0.3022 & -0.0381 & 0.3005 \\
CLIP-I & 0.2834 & 0.1248 & 0.2813 \\
\midrule
\multicolumn{4}{c}{Multi-concept Image Composition (3 models)} \\
Human Raters & 0.5927 & 0.5145 & 0.5919 \\
\midrule
\colorbox{yellow}{M-Sie:GPT-4v} & 0.3209 & 0.3025 & 0.3346 \\
DINO & 0.0979 & -0.1643 & 0.0958 \\
CLIP-I & 0.1512 & -0.0963 & 0.1498 \\
\midrule
\multicolumn{4}{c}{Control-guided Image Generation (2 models)} \\
Human Raters & 0.5443 & 0.5279 & 0.5307 \\
\midrule
M-Sie:GPT-4v & 0.4360 & 0.4975 & 0.3999 \\
\colorbox{yellow}{LPIPS} & 0.3699 & 0.4204 & 0.4133 \\
\bottomrule
\end{tabular} }
\caption{Correlations comparison with existing auto-metrics. We highlight the metric that has the highest overall correlation to humans.}
\label{tab:auto_metrics_corr}
\end{table}


\begin{table*}[!t]
\centering
\scalebox{0.80}{
\begin{tabular}{l|ccc|c|ccc}
\toprule
Metric & M-H$^{SC}_{\text{corr}}$ & M-H$^{PQ}_{\text{corr}}$ & M-H$^{O}_{\text{corr}}$ &  Highest Correlation Image Model & SC$^\text{HCIM}_\text{corr}$ & PQ$^\text{HCIM}_\text{corr}$ & O$^\text{HCIM}_\text{corr}$\\
\midrule
\multicolumn{8}{c}{Text-guided Image Generation} \\
\midrule
Human Raters & 0.5561 & 0.3851 & 0.5057 & SDXL & 0.6635 & 0.5482 & 0.6770\\
\midrule
\multicolumn{8}{c}{Mask-guided Image Editing} \\
\midrule
Human Raters & 0.6063 & 0.5539 & 0.5521 & SDXLInpaint & 0.7883 & 0.6819 & 0.785\\ 
\midrule
\multicolumn{8}{c}{Text-guided Image Editing} \\
\midrule
Human Raters & 0.4663 & 0.5582 & 0.4644 & InstructPix2Pix & 0.7928 & 0.6862 & 0.7860\\
\midrule
\multicolumn{8}{c}{Subject-driven Image Generation} \\
\midrule
Human Raters & 0.5284 & 0.3739 & 0.5102 & DreamBooth & 0.7670 & 0.4084 & 0.7263\\
\midrule
\multicolumn{8}{c}{Subject-driven Image Editing} \\
\midrule
Human Raters & 0.5358 & 0.3099 & 0.5164 & DreamEdit & 0.6726 & 0.2284 & 0.6126 \\
\midrule
\multicolumn{8}{c}{Multi-concept Image Composition} \\
\midrule
Human Raters & 0.6843 & 0.5723 & 0.6828 & CustomDiffusion & 0.9194 & 0.5279 & 0.9112 \\
\midrule
\multicolumn{8}{c}{Control-guided Image Generation} \\
\midrule
Human Raters & 0.6102 & 0.5875 & 0.5911 & UniControl & 0.7025 & 0.7029 & 0.6860 \\
\bottomrule
\end{tabular} }
\caption{Spearman correlation on Human-to.}
\label{tab:human_hcim}
\end{table*}

